Qubit-controlled directional edge states in waveguide QED

We propose an in-situ tunable chiral quantum system, composed of a quantum emitter coupled to a waveguide based on the Rice-Mele model (where we alternate both the on-site potentials and tunnel couplings between sites in the waveguide array). Specifically, we show that the chirality of photonic bound state, that emerges in the bandgap of the waveguide, depends only on the energy of the qubit; a parameter that is easy to tune in many artificial atoms. In contrast to previous proposals that have either shown imperfect chirality or fixed directionality, our waveguide QED scheme achieves both perfect chirality and the capability to switch the directionality on demand with just one tunable element in the device. We also show that our model is easy to implement in both state-of-the-art superconducting circuit and quantum dot architectures. The results show technological promise in creating long-range couplers between qubits while maintaining, in principle, zero crosstalk.

==> fig_Yconfig.tex <==
\newcommand{\combFour}[4]{%U_L (1=high, 0=low), U_R, t_L (1=high, 0=low), t_R,
	\node[draw, circ=8pt] (b) at (0, 0) {};
	\node[below] at (b.south) {$V_\textnormal{C}$};
	\node[draw, circ=8pt] (q) at (0, 0.9) {};
	\node[right] at (q.east) {$V_\textnormal{Q}$};
	\draw[-, line width=0.5pt] (b) -- (q) node [pos=0.5, right]{$t_\textnormal{Q}$};
	\foreach \i in {1,...,3}
	{
		\pgfmathparse{#1 ? "10pt" : "6pt"}
		\edef\Usize{\pgfmathresult}
		\node[draw, circ=\Usize] (a) at (-1.2*\i+0.6, 0) {};
		\node[below] at (a.south) {\ifnum #1=1 $V_\textnormal{R}$ \else $V_\textnormal{L}$ \fi};
		\pgfmathparse{#3 ? "3pt" : "1pt"}
		\edef\tsize{\pgfmathresult}
		\draw[-, line width=\tsize] (b) -- (a);
		\pgfmathparse{#1 ? "6pt" : "10pt"}
		\edef\Usize{\pgfmathresult}
		\node[draw, circ=\Usize] (b) at (-1.2*\i, 0) {};
		\node[below] at (b.south) {\ifnum #1=1 $V_\textnormal{L}$ \else $V_\textnormal{R}$ \fi};
		\pgfmathparse{#3 ? "1pt" : "3pt"}
		\edef\tsize{\pgfmathresult}
		\draw[-, line width=\tsize] (b) -- (a) node [pos=0.5, above] {\ifnum\i=2 $t_\textnormal{2}$ \fi};
	}
	\pgfmathparse{#3 ? "3pt" : "1pt"}
	\edef\tsize{\pgfmathresult}
	\draw[-, line width=\tsize] (b) -- ($ (b) - (0.3,0) $);
	\node[draw, circ=8pt] (b) at (0, 0) {};
	\foreach \i in {1,...,3}
	{
		\pgfmathparse{#2 ? "10pt" : "6pt"}
		\edef\Usize{\pgfmathresult}
		\node[draw, circ=\Usize] (a) at (1.2*\i-0.6, 0) {};
		\node[below] at (a.south) {\ifnum #2=1 $V_\textnormal{R}$ \else $V_\textnormal{L}$ \fi};
		\pgfmathparse{#4 ? "3pt" : "1pt"}
		\edef\tsize{\pgfmathresult}
		\draw[-, line width=\tsize] (b) -- (a) node [pos=0.5, above] {\ifnum\i=2 $t_\textnormal{1}$ \fi};
		\pgfmathparse{#2 ? "6pt" : "10pt"}
		\edef\Usize{\pgfmathresult}
		\node[draw, circ=\Usize] (b) at (1.2*\i, 0) {};
		\node[below] at (b.south) {\ifnum #2=1 $V_\textnormal{L}$ \else $V_\textnormal{R}$ \fi};
		\pgfmathparse{#4 ? "1pt" : "3pt"}
		\edef\tsize{\pgfmathresult}
		\draw[-, line width=\tsize] (b) -- (a);
	}
	\pgfmathparse{#4 ? "3pt" : "1pt"}
	\edef\tsize{\pgfmathresult}
	\draw[-, line width=\tsize] (b) -- ($ (b) + (0.3,0) $);
	\draw[draw=black, dashed] (-0.9,1.25) rectangle (0.9,-0.8);
}

\newcommand{\combFourFinal}[4]{%U_L (1=high, 0=low), U_R, t_L (1=high, 0=low), t_R,
	\node[draw, circ=8pt] (b) at (0, 0) {};
	\node[below] at (b.south) {$V_\textnormal{C}$};
	\node[draw, circ=8pt] (q) at (0, 0.9) {};
	\node[right] at (q.east) {$V_\textnormal{Q}$};
	\draw[-, line width=0.5pt] (b) -- (q) node [pos=0.5, right]{$t_\textnormal{Q}$};
	\foreach \i in {1,...,3}
	{
		\pgfmathparse{#1 ? "10pt" : "6pt"}
		\edef\Usize{\pgfmathresult}
		\node[draw, circ=\Usize] (a) at (-1.2*\i+0.6, 0) {};
		\node[below] at (a.south) {\ifnum #1=1 $V_\textnormal{R}$ \else $V_\textnormal{L}$ \fi};
		\ifnum \i=1
		\draw[-, line width="1pt"] (b) -- (a);
		\else
		\draw[-, line width="3pt"] (b) -- (a) node [pos=0.5, above] {\ifnum\i=2 $t_\textnormal{2}$ \fi};
		\fi
		\pgfmathparse{#1 ? "6pt" : "10pt"}
		\edef\Usize{\pgfmathresult}
		\node[draw, circ=\Usize] (b) at (-1.2*\i, 0) {};
		\node[below] at (b.south) {\ifnum #1=1 $V_\textnormal{L}$ \else $V_\textnormal{R}$ \fi};
		\draw[-, line width="1pt"] (b) -- (a);
	}

	\pgfmathparse{#3 ? "3pt" : "1pt"}
	\edef\tsize{\pgfmathresult}
	\draw[-, line width=\tsize] (b) -- ($ (b) - (0.3,0) $);
	\node[draw, circ=8pt] (b) at (0, 0) {};
	\foreach \i in {1,...,3}
	{
		\pgfmathparse{#2 ? "10pt" : "6pt"}
		\edef\Usize{\pgfmathresult}
		\node[draw, circ=\Usize] (a) at (1.2*\i-0.6, 0) {};
		\node[below] at (a.south) {\ifnum #2=1 $V_\textnormal{R}$ \else $V_\textnormal{L}$ \fi};
		\ifnum \i=1
		\draw[-, line width="1pt"] (b) -- (a);
		\else
		\draw[-, line width="3pt"] (b) -- (a);
		\fi
		\pgfmathparse{#2 ? "6pt" : "10pt"}
		\edef\Usize{\pgfmathresult}
		\node[draw, circ=\Usize] (b) at (1.2*\i, 0) {};
		\node[below] at (b.south) {\ifnum #2=1 $V_\textnormal{L}$ \else $V_\textnormal{R}$ \fi};
		\pgfmathparse{#4 ? "1pt" : "3pt"}
		\edef\tsize{\pgfmathresult}
		\draw[-, line width="1pt"] (b) -- (a) node [pos=0.5, above] {\ifnum\i=2 $t_\textnormal{1}$ \fi};
	}
	\pgfmathparse{#4 ? "3pt" : "1pt"}
	\edef\tsize{\pgfmathresult}
	\draw[-, line width=\tsize] (b) -- ($ (b) + (0.3,0) $);
	\draw[draw=black, dashed] (-0.9,1.25) rectangle (0.9,-0.8);
}

\begin{tikzpicture}[
	circ/.style = {circle, minimum size=#1,
		inner sep=0pt, outer sep=0pt}
	]
	
	\combFourFinal{0}{1}{0}{0};
	
\end{tikzpicture}
